Track Extraction with Hidden Reciprocal Chain Models

This paper develops Bayesian track extraction algorithms for targets modelled as hidden reciprocal chains (HRC). HRC are a class of finite-state random process models that generalise the familiar hidden Markov chains (HMC). HRC are able to model the "intention" of a target to proceed from a given origin to a destination, behaviour which cannot be properly captured by a HMC. While Bayesian estimation problems for HRC have previously been studied, this paper focusses principally on the problem of track extraction, of which the primary task is confirming target existence in a set of detections obtained from thresholding sensor measurements. Simulation examples are presented which show that the additional model information contained in a HRC improves detection performance when compared to HMC models.

==> MB_construction_lbw.tex <==

Consider a random process $\{X_t\} $ %= \lbr X_1, \ldots, X_T \rbr$ 
indexed by $t \in \{0, 1,\ldots, T\} $ for some fixed integer $T \geq 2$. 
The index $t$ will denote an index on a set of event epochs. 
At each epoch $t$,  the random variable $X_t$ takes a value on a finite state space $\Sc = \{1,\ldots, N\}$, where $N \geq 2$ is a fixed integer.
The process $\{X_t\}$
is said to be {\it reciprocal} \cite{Jami74}, if 
\begin{eqnarray}
\Pr \lbr X_t | X_s, \forall \, s \neq t \rbr & = & \Pr \lbr X_t | X_{t-1},
X_{t+1} \rbr \ ,
\label{eq:rp1}
\end{eqnarray}
for each $t = 1, \ldots, T-1$. Thus $X_t$ is conditionally independent
of $X_0, \ldots, X_{t-2}, X_{t+2}, \ldots, X_T$ given its neighbours
$X_{t-1}$ and $X_{t+1}$. The reciprocal model is specified by the set of three-point
transition functions \eqref{eq:rp1} together with a given joint
distribution on the end points $\Pr \lbr X_1, X_T \rbr$. 
A reciprocal process is a one-dimensional Markov random field, although is not, in general, a Markov process. However all Markov processes are reciprocal \cite{Jami74}.
Denote the three-point transition functions in (\ref{eq:rp1}) by
\begin{eqnarray}
Q_{i,j,\ell}(t) = \Pr \lbr X_t = j | X_{t-1}= i, X_{t+1} =
\ell \rbr),  \label{eq:3pt_tr}
\end{eqnarray}
for $i,j,\ell \in \Sc$, $t=0, \ldots, T-1$, and the end-points distribution given by
\begin{eqnarray}
\Pr \lbr X_0=i, X_T=j \rbr & = & \Pi_{i,j}, \quad i,j \in \Sc \ .
\label{eq:end_pts}
\end{eqnarray}
Pinning the end point of a RC generates a Markov bridge, which we consider to be a Markov process with the end point $X_T$ fixed to a specified value, together with the initial marginal distribution, derived from \eqref{eq:end_pts}, that corresponds to the value $X_T$ takes. The term bridge generally refers to a process with specified values at both start and end times, however the use of the term can vary (see Section \ref{ssec:term} for a comment on terminology).

So for the finite ($N$) state case, a RC can be
regarded as $N$ Markov bridges, one corresponding to each of the
possible final states taken by $X_T$. The important role of Markov bridges becomes apparent when we consider the joint distribution of the states of a RC, using direct Bayes' conditioning and \eqref{eq:rp1},
\begin{eqnarray}
\Pr \lbr X_0, \ldots, X_T \rbr = \Pr \lbr X_1, X_T \rbr \lb \prod_{t=2}^{T-1} \Pr \lbr X_t |
X_{t-1},X_T \rbr \rb .
\label{eq:RC_like}
\end{eqnarray}
The terms contained within the product in \eqref{eq:RC_like} are precisely the state transitions for a MB pinned at $X_T$, and depend only on the three-point transitions \eqref{eq:3pt_tr}. Based on the properties of a RC a
backwards recursion was obtained in \cite{WC11} which fully specifies the set of $N$ MB transitions for $t=T-2,T-3, \ldots,
1$ via
\begin{eqnarray}
B_{i,j}^k(t) & = & \Pr \lbr X_{t+1} = j | X_t = i, X_T = k \rbr \nonumber \\ &=&  \frac{Q_{i,j,\ell}(t+1)}{B_{j,\ell}^k(t+1)} \lb 
\sum_{m=1}^{N} \frac{Q_{i,m,\ell}(t+1)}{B_{m,\ell}^k(t+1)} \rb^{-1}
,\  \label{eq:MBform2}
\end{eqnarray}
the last term on the right being the normalisation constant. Initialisation
is with $B_{i,j}^k(T-2) = Q_{i,j,k}(T-1)$. The quantity
on the right hand side of equation \eqref{eq:MBform2} is independent of the index
$\ell$. Now since the terms
$B_{j,.}^k(t+1)$ form a probability distribution (i.e. they are
non-negative and sum to unity) for each $i,k$ and $t$, there is at
least one index $\ell$ for which $B_{j,\ell}^k(t+1)$ is non-zero. So
this index may be selected on the rhs of \eqref{eq:MBform2}, and thus
\eqref{eq:MBform2} is well defined. From a numerical perspective, it
may thus be appropriate to choose a value of $\ell$ (for each $j,k, t$) which
maximises the value of $B_{j,\ell}^k(t+1)$ when performing the calculations in \eqref{eq:MBform2}.  Determining the set of MBs from
the specified three point transitions requires complexity of
$O(N^3T)$, i.e. $O(N^2T)$ for each MB. The Markov bridge with final state $k$ has an initial
probability distribution $\pi^k_i$ given by the conditional
distribution
\begin{eqnarray}
\pi^k_i & = & \Pr \lbr X_0 = i | X_T = k \rbr \ = \ \frac{\Pi_{i,k}}{\sum_{j=1}^N \Pi_{j,k}} \ .
\label{eq:MBinit}
\end{eqnarray}
Thus we have that any RC may be uniquely specified by the
finite set of Markov bridges with probability transition matrices
given by \eqref{eq:MBform2} and initial distributions
\eqref{eq:MBinit}. 
%As mentioned in \cite{WC11} the final state $X_T$ is {\it not} governed by Markov transitions, an issue raised by Jamison in \cite{Jami74} (Sec. 4). However, in Sec. \ref{sec:filt}, we avoid this issue by deriving filters for the joint process $(X_t,X_T)$, which is the approach of \cite{CW12}. Indeed, \cite{CW12} proves that this joint process is Markovian with transitions governed by the MB transitions \eqref{eq:MBform2}, a property we will exploit in deriving the optimal filter for HRC, and in turn detectors.
As we will see below, a more intuitive description of RCs can be found via the construction of a reciprocal process from a Markov process, which we will refer to as the {\it base process}. This construction was established in \cite{Jami74} and will be used here, as it was in \cite{WC11}, for numerical simulations in Section \ref{sec:sims}.



==> filters_lbw.tex <==
Consider first a HRC $\Yc$, observed in a clutterless environment, with state $\Xc$, known MB transition probability matrices  $B_{i,j}^k(t)$,  $t=0,2,\ldots, T-2$,  and known  observation probabilities $C_i(t), t = 0,\ldots, T, i = 1, \ldots, N$. 
Given a sequence of observations, $Y_0,\ldots,Y_T$, the aim here is to compute the filtered {\it a posteriori} probability (APP) mass functions
\begin{align}
q_{i}(t)  & =  \Pr \lbr X_t = i | Y_1, \ldots, Y_t \rbr \ ,
\label{eq:filtRC_def}
\end{align}
for each $t=0,\ldots, T-1$, and each $i=1,\ldots,N$. These APPs can be calculated from the individual bridge APPs, $q_i^k(t)$, for each $k = 1, \dots, N$,
\begin{align}
q_{i}(t) =  \sum^N_{k=1} \Pr \lbr X_t = i, X_T = k | Y_1, \ldots, Y_t \rbr =  \sum^N_{k=1} q_{i}^{k}(t) \ ,
\label{eq:filt_def}
\end{align}
via the law of total probability. Analogously to the hidden Markov model filter (see e.g. \cite{EM02}), it is easily shown via Bayes' rule that $q_i^k(t)$ can be evaluated recursively, for $t=1,\ldots, T-1$ by 
\begin{align}
q_{i}^{k}(t) & = \frac{C_i(t) \, \sum_{j=1}^N B_{j,i}^k(t-1) \, q_{j}^{k}(t-1)}{h(t)} \ ,
\label{eq:std_filt}
\end{align}
where the normalising term is
\begin{align*}
h(t) & =  \Pr \lbr Y_t | Y_0, \ldots, Y_{t-1} \rbr \\
 & = \sum_{i,k=1}^N C_i(t) \, \sum_{j=1}^N B_{j,i}^k(t-1) \, q_{j}^{k}(t-1) \ .
\end{align*}
The overall computational cost of the above filtering recursions is $O(N^3T)$. Initialisation at $t=0$ is via
\begin{align*}
q_{i}^{k}(0) = \frac{C_0(i) \, \Pi_{i,k}}{h(0)},
\end{align*}
\begin{align*}
\mathrm{where}\ \ h(0) = \Pr \lbr Y_0 \rbr = \sum_{i,k=1}^N C_0(i) \, \Pi_{i,k} .
\end{align*}
At each time $1 \leq t \leq T-1$, we can produce the marginal APPs $\Pr \lbr X_t | Y_0, \ldots, Y_t\rbr$ (i.e. a filtered estimate for $X_t$) and $\Pr \lbr X_T | Y_0, \ldots, Y_t\rbr$ (i.e. a predicted estimate for $X_T$). The filtered estimate for the final point is obtained via
\begin{align*}
q^{k}(T) & = \frac{C_T(k) \, \sum_{i=1}^N q_{i}^{k}(T-1)}{h(T)},\\ 
 \mathrm{where} \ \ h(T) & = \Pr \lbr Y_T | Y_0, \ldots, Y_{T-1} \rbr \\
& = \sum_{i,k=1}^N C_T(k) \, q_i^k(T-1) \ .
\end{align*}
The observation log-likelihood can be evaluated via $\log \Pr \lbr Y_0, \ldots, Y_T \rbr = \sum_{t=0}^T \log h(t)$. 
This approach avoids any potential numerical underflow issues which might arise if the {\it conditional} (un-normalised) MB filters as defined in \cite{WC11} were used. A track extraction type algorithm can be obtained by comparing the log sequence likelihood to a threshold.


\subsection{Optimal Single Observation Filter with Clutter \label{ssec:single_obs_filt}}
If we now consider the case where there is clutter present, we can show that the complexity does not increase for the detection problems posed above by assuming certain conditions on the clutter process. We derive a recursion using the single observation model properties \eqref{eq:singl_obs_defn},

\begin{figure*}[t]
\normalsize
\begin{align*}
q^{k}_{i}(t)  & =  \Pr \lbr X_t = i, X_T = k| Y_0, \ldots, Y_t \rbr \\
&= \frac{ \sum_{j=1}^N \Pr \lbr X_t = i, X_T = k, U_t = j, Y_t | Y_0, \ldots, Y_{t-1} \rbr}{\Pr \lbr Y_t | Y_0, \ldots, Y_{t-1}  \rbr}\\
&= \frac{ \sum_{j=1}^N \Pr \lbr Y_t | X_t = i, U_t = j \rbr\Pr \lbr X_t = i, X_T = k, U_t = j | Y_0, \ldots, Y_{t-1} \rbr}{\Pr \lbr Y_t | Y_0, \ldots, Y_{t-1} \rbr}\\
&= \frac{ \sum_{j=1}^N \big( (1-\epsilon)C_i(t) + \epsilon C_j(t) \big) \Pr \lbr X_t = i, X_T = k | Y_0, \ldots, Y_{t-1}\rbr \Pr \lbr U_t = j \rbr}{\Pr \lbr Y_t | Y_0, \ldots, Y_{t-1} \rbr}\\
&= \frac{   \sum_{j=1}^N \Pr \lbr U_t=j \rbr\big( (1-\epsilon) C_i(t) + \epsilon C_j(t) \big) \sum_{l=1}^N B_{l,i}^k(t-1) \, q_{l}^{k}(t-1)}{d(t)}\\
\end{align*}
% Restore the current equation number.
% IEEE uses as a separator
\hrulefill
% The spacer can be tweaked to stop underfull vboxes.
\vspace*{4pt}
\end{figure*}
for each $t=0,\ldots, T-1$, and each $i,k=1,\ldots,N$, and noting that the given sequence of observations, $Y_0,\ldots,Y_T$, may be clutter generated. The derivation above has made use of the law of total probability, conditional probability, property \eqref{eq:cond_ind}, definition \eqref{eq:singl_obs_defn} and the reciprocal property \eqref{eq:rp1}. If we assume the clutter process is not time varying and spatially uniform, we can simply the expression above,

\begin{figure*}[t]
%\normalsize
\begin{align*}
q^{k}_{i}(t)  &= \frac{\big((1-\epsilon) C_i(t) + \epsilon\frac{1}{N}\sum_{j=1}^N C_j(t) \big)  \sum_{\ell=1}^N B_{\ell,i}^k(t-1) \, q_{\ell}^{k}(t-1)  }{d(t)}\\
\end{align*}
% Restore the current equation number.
% IEEE uses as a separator
%\hrulefill
% The spacer can be tweaked to stop underfull vboxes.
%\vspace*{4pt}
\end{figure*}

This is a similar expression to that of the clutter-free model; only the observation part of the model has changed, which demonstrates there is no increase in complexity. 
%We should point out that, since no analytic form for the probability distribution of the sequence log likelihood under the null hypothesis (no target present) can be found, numerical approaches (such as simulations) are required in order to sensibly set the detection threshold. 



==> intro_lbw.tex <==
\subsubsection{Problem Description}
Track extraction is a statistical hypothesis testing technique that tests for the presence of a dynamic target in a set of detections of uncertain origin that are obtained from a detector applying a low threshold to sensor measurements \cite{vK, WK}. While standard multiple hypothesis tracking (MHT) algorithms confirm or delete tracks based on the likelihood of individual candidate tracks \cite{Blackman}, track extraction algorithms use the entire set of detections to first decide whether a target exists, with the likelihood supplied by applying a tracker with an underlying model of target dynamics. It is therefore also a detection process, with quantities such as detection probability and false alarm rate, but works on a higher level of abstraction than a sensor detector, leading to tracks rather than potentially unrelated point estimates. Classically, tracking and track extraction algorithms apply the Markov assumption to the target dynamics. At finer time scales the assumption is generally appropriate, and many well-known Markov based tracking algorithms are discussed in the literature \cite{Blackman}-\cite{BP}. This paper is motivated by applications with coarser time scales where the Markov assumption is less valid generally because real-world targets have a defined origin and destination. We will call such targets {\it source-destination aware}, and we will examine whether the use of dynamic target models which incorporate such information can improve track extraction.\\

%There have been various approaches to target behaviour modelling for tracking, incorporating notions of defined manoeuvres or of progression between destinations according to some intent [x]-[x]. While the motivation for these works is inference, such as anomaly detection, it is assumed rather than shown that a more complex model improves tracking performance as compared to some equivalent but behaviour-naive model. More specifically, it is implicitly assumed that a) there is a target present and b) the target has intent. 

%This paper focuses explicitly on how modelling the intent of targets can improve tracking as compared to naive tracking models. Thus we consider targets in a TBD setting that move according to a simple model of intent that is substitutable for the standard Markov models, which we call ``source-destination awareness''.
\subsubsection{Related Work}
From a modelling point of view, being source-destination aware means that the initial and final target states have a specified joint probability distribution and that target dynamics are anticipative, or non-causal, reflecting the intention of the target to move towards its destination. There have been a range of approaches to incorporating available \emph{a priori} information about the future within the class of Markov models, both at the estimation stage and in the target dynamics model itself. Both methods amount to ``back propagating'' the influence of a future state value or distribution by appropriate conditioning. For example in \cite{CLW85}-\cite{KP}, \emph{a priori} destination information is incoproated via a corrective term into the state update of continuous-time Gauss-Markov processes, and specifying an \emph{a priori distrubition} for a future time of the state process creates a new Markovian process referred to as a Schr\"{o}dinger bridge \cite{Jami75}-\cite{GP}. What is however not able to be modelled within the Markovian class is the future information that is conditional on the past state of the system (the intention to proceed between a source and associated destination). The injection of a relationship between future and past states other than that induced by the evolution of the “globally naive” first order Markovian dynamics, adds a probabilistic dependence that raises the class of model to what is known as the class of {\it reciprocal processes}. Reciprocal processes were studied in detail by Jamison \cite{Jami74} in a general setting, and subsequently by Levy {\it et al} \cite{LFK90} who considered the realisation and state estimation problem for the Gaussian discrete parameter case. There are many other related works which are summarised in \cite{WC11}, to which to the interested reader is referred for more background. \\

Reciprocal chains (RCs) are finite-state reciprocal processes, and hidden reciprocal chains (HRCs) are stochastic processes generated from an RC via some noisy and/or incomplete observation mechanism, analogous to hidden Markov chains (HMC). We work with finite-state processes because the arbitrary source-destination pair relationships that are relevant to tracking on courser time scales (such as between airports) are better captured by a cellular state space. Finite states also allow for more abstract target attribute states. We thus recount the present state of development in inference of HRCs; un-normalised optimal filters/smoothers for HRC, derived using a Bayesian approach, were presented in \cite{WC11}. Normalised filters and smoothers were developed in \cite{CW12}, which also considered a generalisation of HRC to incorporate ``waypoints'' on the target trajectory. Maximum likelihood estimation of state sequences (MLSE) for HRC was presented in \cite{WV13}. In \cite{FK13},\cite{FKW11} an approach called destination aware tracking based on HRC was first proposed, but the RC models tested, being pinned to a single destination, in fact remained in the Markov class. Thus the tracking performance of non-causal HRCs has not been studied in detail. The present paper is an extension of the work presented in \cite{SDW}, which provided an intuitive description of how HRCs may be applied in a target tracking problem. The filtering algorithms derived in this paper proceed in the manner of the Bayesian decomposition of a reciprocal chain into a collection of end-pinned bridge processes that was established in \cite{WC11}.

\subsubsection{Contributions}

The track extraction setting to which we introduce the new model, and compare to existing models, is similar to the setup in \cite{vK}, with two key differences. Firstly, we perform optimal Bayesian estimation over finite states, rather than a continous space, and secondly we operate on a fixed interval rather than in an online context, though the likelihood ratio test here has the same form as the sequential probability ratio test of \cite{vK}. To recreate the setting, we include two types of uncertainty, the presence of ‘clutter’ - detections that do not originate from the target, and the usual `sensor' noise on position estimates. In section V of \cite{vK} signal-strength information is used and improves the track extraction performance, but without loss of generality we remove any notion of SNR and signal amplitude to emphasise the role of the model in differentiating clutter from target detections, since this is equivalent to treating all detections as having equal likelihood of originating from either clutter or target. Observation models for two representative track extraction regimes are developed and tested. In each there is at most one target during the tracking interval. In the first we process one sensor return at each time increment, with a certain chance that the return is clutter generated (sensor returns could here be conceived as erroneous outputs from a fast-time tracker, such as particle filter or EKF). In the second scenario we allow multiple measurements at each time, with at most one due to the target and all others clutter generated, a scenario also typical in visual tracking and which is very similar to the observation model of \cite{vK}. A dynamic model of the target is constructed which incorporates target dynamics, including the global source-destination attributes. The likelihood associated with a given set of detections is evaluated using the new class of normalised hidden reciprocal chain (HRC) filters. This likelihood forms the basis for a target extraction algorithm.\\

The key contributions made in this paper is in answering the question of whether modelling the source-destination awareness of a target can improve tracking, and to what extent the tracking is improved, as a function of the parameters of a HRC, which can model source-destination awareness. With most finite data non-linear inference problems, it is infeasible to obtain {\it a priori} performance metrics, so we are led to the use of numerical simulations to study the performance of the new algorithms proposed here. The contributions and numerical study we present here are significant as there has been a recent shift towards analyst support software, due to increasing data rates and the inability for human analysts to process the volumes of information. There have been many approaches from the machine learning and computer vision fields in this direction, focusing on higher level inference tasks such as anomaly detection. However these approaches assume rather than shown that modelling intent improves tracking, which this paper focuses on explictly using the track extraction setting.

\subsubsection{Paper Outline}

 The layout of the paper is as follows: in section II, we define HRC and summarise the pinned Markov process construction of an HRC such as given in [6]. The observation models are defined in section III before the normalised optimal filters are derived described in section IV, and the corresponding detectors in section V. Numerical simulations are presented in section VI, before we conclude in VII with a discussion of future research directions.


